Improving Faithfulness of Abstractive Summarization by Controlling Confounding Effect of Irrelevant Sentences

Lack of factual correctness is an issue that still plagues state-of-the-art summarization systems despite their impressive progress on generating seemingly fluent summaries. In this paper, we show that factual inconsistency can be caused by irrelevant parts of the input text, which act as confounders. To that end, we leverage information-theoretic measures of causal effects to quantify the amount of confounding and precisely quantify how they affect the summarization performance. Based on insights derived from our theoretical results, we design a simple multi-task model to control such confounding by leveraging human-annotated relevant sentences when available. Crucially, we give a principled characterization of data distributions where such confounding can be large thereby necessitating the use of human annotated relevant sentences to generate factual summaries. Our approach improves faithfulness scores by 20\% over strong baselines on AnswerSumm \citep{fabbri2021answersumm}, a conversation summarization dataset where lack of faithfulness is a significant issue due to the subjective nature of the task. Our best method achieves the highest faithfulness score while also achieving state-of-the-art results on standard metrics like ROUGE and METEOR. We corroborate these improvements through human evaluation.

==> src/analysis.tex <==
\section{Analysis}
This section further explores performance of our models on various ancillary objectives. First, we consider performance on extracting relevant sentences.
\subsection{Extractive Answer Summarization}
As previously described, we treat relevant sentence extraction from each answer as an extractive answer summarization task. In the RoBERTa model, we pass each answer separately to the model concatenated with the question as input to predict the relevant sentences in that answer. We add the \texttt{CLS} token before each sentence and use its representation to predict whether a sentence in the answer is relevant. We generate the extractive summary for the RoBERTa model by concatenating the predicted relevant sentences across all answers. Model selection during training is done to maximize ROUGE-1 score of the extractive summaries against concatenation of gold relevant sentences, similar to the SURE-Summ model. Table \ref{tab:rel_sent_pred} shows the performance
of the RoBERTa model for extracting relevant sentences. We see that the SURE-Summ model with the multi-task objective improves upon the RoBERTa model by 6-7\%. However, the absolute scores for both RoBERTa and the SURE-Summ model are low pointing to the difficulty of selecting relevant sentences in the \answersumm{} dataset. The UNSURE-Summ model on the other hand achieves high relevant sentence prediction accuracy since it predicts distantly supervised relevant sentences and not gold relevant sentences. This shows that predicting sentences that have high overlap with the summary are easier
\input{tables/relevant_sent_results}

Table \ref{tab:gold_vs_distant} shows the overlap between gold relevant sentences and those obtained using distant supervision at various ROUGE-1 thresholds. At every threshold value, the number of false positives is quite high in relation to the true positives. Because irrelevant sentences can have high overlap with the final summary in terms of ROUGE scores, they can act as confounders when learning an abstractive summarization model over the full answers.
\input{tables/gold_vs_distant_relevant}

\begin{comment}
\subsection{Qualitative Analysis}
Figure \ref{fig:example_predictions} shows two example predictions of the SURE-Summ-BART model drawn from five predictions with highest and lowest faithfulness scores respectively. We see that in both cases the SURE-Summ-BART model's predictions are more multiperspective. In the first example BART's prediction is very poor. In the second example BART's prediction is of comparable quality to the SURE-Summ-BART model, however the latter's prediction includes all the perspectives that are in the gold summary while BART's prediction is missing one perspective (tapioca).
\input{tables/example_predictions}
\end{comment}

==> src/intro_old.tex <==
\Blue{
\begin{itemize}
    \item We look at extract-and-generate or extractive-abstractive (EA) summarization through a new lens. Previously EA models have been proposed to address summarizing long inputs but we theoretically and empirically demonstrate how EA models can improve faithfulness even when the inputs are not long.
    \item The starting point of our work is that the generation probability (or likelihood) of seq2seq models is indicative of hallucination or lack thereof. This is the assumption behind BARTScore: “evaluation of text through the lens of its probability of being generated” with higher probability indicating higher quality of generated text with less hallucinations. BARTScore has been shown to achieve higher correlation with human judgements of faithfulness.
    \item Many query based summarization datasets are obtained using an annotation pipeline where human annotators first identify a subset of sentences (or phrases) in document that is relevant to the query and then abstractively summarize the relevant sentences. In such settings the final summary is \textit{causally independent} of the irrelevant sentences given the relevant sentences. Note that causal independence is different from statistical independence \cite{ay2008information}.
    \item Towards that end, we look at extract-and-generate summarization through the framework of causal mediation analysis (CMA). CMA aims to separate direct and indirect effects of the treatment (input) from the outcome (output) through mediator variables. Applying it to summarization we separate the \textit{indirect effect} of the irrelevant sentences on the summary. 
    \item Previous work (\TODO{cite CoCo paper}) has studied the causal effect of language prior on the final summary which they claim is a reason for hallucination. However, hallucination can occur even when a summarization model relies on the provided input to generate the final summary; for example in Figure 1 the  BART model combines information from two different answers “keep[ing] all food sealed in plastic containers” and “Sealing basement window cracks with silicone” to generate the summary “cover holes with plastic’’ which is not faithful since the answers suggest covering/sealing holes with silicone and not plastic. In this example the first sentence is marked as irrelevant while the second sentence is marked as relevant by human annotators and the bold words emphasize textual overlap. 
    \item While the precise mechanism in which abstractive summarization models combine information to generate a summary is unknown, we hypothesize that learning an abstractive summarization model directly from the whole input when the true summary was generated by human annotators from a small subset of the input causes the model to learn spurious associations between summary terms and terms in irrelevant sentences.
    \item We quantify causal effect of irrelevant sentences on the final summary using information flow --- a concept that has been used in the statistics literature to quantify direct and indirect causal effects in the context of mediation analysis.
    \item We show that the magnitude of the indirect effect is proportional to the entropy of relevant sentences under the true data distribution. Therefore, in datasets like AnswerSumm where there is significant subjectivity in determining which sentences are relevant, the indirect effect of irrelevant sentences on the final summary is large.
    \item Our main contribution is to precisely characterize how the indirect effect affects abstractive summarization. We show that the risk (expected negative log-likelihood under the true data distribution) of the optimal predictor trained to generate the final summary from the whole input is always greater than the risk of the predictor trained to generate the final summary from the true relevant sentences. The difference in risk is precisely the magnitude of the indirect effect (of the irrelevant sentences).
    \item Our theoretical results shed light on when extract-and-generate models should be prefered over direct models and viceversa. In datasets where there is high uncertainty in selecting relevant sentences, it is imperative to train abstractive summarization models from true relevant sentences to improve faithfulness. On the other hand when relevant sentences can be predicted with high certainty, e.g. if the relevant sentences are almost always at the beginning of a document, then indirect effect of the irrelevant sentences is small and training a model that directly summarizes the input should suffice. 
    
    \item Since at test time relevant sentences are not known, we also need a relevant sentence extractor whose output is passed to the generator. This however results in one problem: exposure bias, wherein at test time the generator sees predicted relevant sentences instead of gold relevant sentences. Towards that end we train a single model that performs both relevant sentence selection and summary generation with different prefixes. Since the parameters between the two stages are shared this reduces exposure bias and our model achieves the best test log-likelihood scores of all models. Our model also achieves significantly higher faithfuless scores are evaluated by BARTScore which we adapt to our setting.
\end{itemize}
}

Although community question answering (CQA) platforms like Quora, Stack Exchange, and Facebook groups enable online users to quickly get answers to their questions on a broad range of topics, the amount of often redundant information can be overwhelming. Query-based answer summarization (QAS) \cite{tomasoni2011metadata,fabbri2021answersumm} aims to improve user experience by surfacing a \emph{diverse} set of \textit{relevant} perspectives across answers in a single succinct \textit{abstractive summary} that is \emph{faithful} to the original answers. 
However, existing methods are still far from achiving the goal.

%The rise of community question answering (CQA) platforms like Quora, Stack Exchange, Reddit, and Facebook groups among others, has enabled online users to quickly find answers to questions on a broad range of topics. The overwhelming amount of redundant information
%is a major problem in such forums, where often times a new user question can be answered from information contained in answers to similar questions. This calls for AI systems that succinctly summarize answers to similar questions. It is therefore desirable for such automatically generated summaries to be faithful to the original answers including diverse perspectives from the answers.
%In this paper, we study the task of  query-based answer summarization (QAS) in the context of CQA and investigate different approaches.

\paragraph{The need for new methods for QAS.}
%Despite sharing many features from question answering and multi-document or long text summarization tasks, the QAS task presents unique challenges. Unlike question answering which usually involves generating a single answer to a given question, in QAS there usually exists multiple valid answers for a question. And in contrast to standard summarization tasks where the most salient information from the input text is summarized, a generated summary in the QAS task may combine multiple salient and potentially contradictory opinions into a single multi-perspective summary. 
Neural language models such as BART \citep{lewis2020bart} or T5 \citep{raffel2019exploring} which perform well on standard QA and summarization tasks, struggle to summarize multiple opinions faithfully. This is due to several challenges that are unique to the QAS task like combining multiple salient and potentially contradictory opinions into a single multi-perspective summary and the 
existence of multiple valid answers for a given question.
Figure \ref{fig:example} shows an example from the \answersumm{} dataset \cite{fabbri2021answersumm}, where the BART generated summary misses several perspectives and also suffers from subtle intrinsic hallucination (see Appendix \ref{app:dataset_details} for details).
To improve factuality and coverage of generated summaries, \citet{fabbri2021answersumm} proposed using entailment-based and semantic area based rewards in a reinforement learning (RL) framework. However, they do not address the long input problem in answer summarization, nor do they specifically evaluate multiperspectivity and faithfulness of generated summaries. Instead, they merely report ROUGE and NLI scores --- metrics which are known to correlate poorly with human judgements of factuality~\citep{gabriel-etal-2021-go, falke2019ranking}. 
In this paper, we propose to address these challenges using a novel extractive-abstractive summarization approach, grounded in strong theoretical foundations and empirical demonstrations. The main idea of our approach is that extractive-abstractive summarization can improve faithfulness regardless of the length of the input. We develop a simple and yet novel extractive-abstractive model for answer summarization and perform rigorous evaluation of our models including human evaluation.
We also find that with further tuning, the baselines in~\citet{fabbri2021answersumm} yield significantly higher ROUGE scores, which outperform their RL based method. 


%\asli{I don't think we motivated why we need to use extractive-abstractive summarization. Why do we think Fabbri's method is not enough for instance? We need to motivate two things which is supposedly different than Fabbri's specifically the miltiperspectivity and faithfullness here to align with the paper title!}
%\asli{put an example instance with baseline model generation with failures}. 
%\asli{Now, in a few sentences say a few things about how previous work have approached this problem. If no previous work, then start talking about the new proposal since we already mentioned baseline LMs fail at this task.}


\noindent{\textbf{Extractive-Abstractive (EA) answer summarization}} 
is posed as a natural model to address long document summarization in earlier work \cite{chen-bansal-2018-fast, mao2021dyle} with no technical justification beyond handling long inputs. We present the first theoretical justification for EA summarization as a means for improving faithfulness regardless of input length. Specifically, we show that if the input contains a small number of relevant sentences such that the summary is conditionally independent of the input given relevant sentences --- e.g. in \answersumm{} \citep{fabbri2021answersumm} and \textsc{QMSum} datasets \cite{zhong2021qmsum}, annotators first extract relevant sentences or phrases for the given query and then summarize the relevant sentences --- then EA models can be designed that are provably more faithful than models that directly generate the final summary from the original input.
%\asli{next sentence is too long.}
%One of our main contribution is conceptual where we show that in the \answersumm{} \citep{fabbri2021answersumm} setting where the final summary is conditionally independent of the answers given relevant sentences, then under practical assumptions, abstractive summarization models that are trained to generate the summary from relevant sentences are provably more faithful than models that are trained to directly generate the summary from the answers. 
We measure faithfulness using \bartscore{} \citep{yuan2021bartscore} adapted to our setting, which has been shown to correlate better than other metrics on human factuality scores. Empirically, we show that a BART model trained to generate the final summary from golden relevant sentences but uses full answers at test time improves faithfulness by 43\% over the standard BART model.

\noindent{\textbf{Multi-task seq2seq model.}}
Building on the above result, we propose SURE-Summ, a \emph{supervised}-\emph{repeated-summarization} approach similar to \textit{extract-and-generate} methods \citep{chen-bansal-2018-fast} for multi-answer summarization. Specifically, given the question, our model extracts relevant sentences from each answer and then summarizes the extracted sentences to generate the final summary. However, in contrast to previous approaches, we view the ``extraction'' and ``generation'' components as separate summarization tasks and formulate repeated summarization as a single multi-task seq2seq model. 
%Our model summarizes each answer independently in an extractive fashion, and then summarizes all the intermediate summaries to produce the final summary in an abstractive fashion. 
The unified seq2seq formulation enables efficient multi-task transfer between the two tasks and, unlike previous extract-and-generate models, does not require careful selection of sparsity parameters \cite{paranjape-etal-2020-information, li-etal-2021-ease, mao2021dyle}. Our approach also eschews RL \cite{chen-bansal-2018-fast}, which may suffer from high variance and training instability issues \cite{mao2021dyle}. An unsupervised version of our model (UNSURE-Summ) that does not use gold relevant sentence annotations during training  also improves faithfulness of generated summaries.

\noindent{\textbf{Rigorous evaluation.}}
To evaluate model output summaries from \emph{multiperspectivity} aspect, we introduce a new Perspective Score leveraging human-annotated perspectives in the golden summaries from the \answersumm{} dataset. Since SURE-Summ model is trained to generate abstractive summaries from gold relevant sentences while also identifying relevant sentences, it improves faithfulness scores by 20\% over the standard BART baseline, METEOR score by 5.4\%, and our Perspective scores by 3.5--5.8\%. Lastly, we show that our reformulated \bartscore{} has the highest correlation with human factuality judgements as compared to all other metrics. The SURE-Summ model matched or exceeded the BART baseline on 72\% and 70\% of examples, respectively on faithfulness and multiperspectivity of generated summaries as evaluated by humans. %Faithfulness was multiperspectivity was strictly better than BART on 53\% and 57\% of examples respectively.

%Finally, we explore standard pipeline models with separately trained extractor and generator models which ensures conditional independence of the final summary from the answers given the relevant sentences. As a result pipeline models significantly improve faithfulness and multi-perspectiveness of the generated summaries over a single model at the cost of doubling up the number of parameteres. Our best model for the \answersumm{} dataset uses the SURE-Summ model as the extractor and BART as the generator improving almost all metrics over the BART baseline.
%\input{tables/example_cluster_summaries}

%Using the Sure-Summ model as the extractor and a BART model as generator in a pipeline model achieves 1-2\% improvement on Rouge 1/2 scores over the BART baseline, while improving faithfulness scores by around 50\%, perspective scores by 10.5 to 14.4\%, and Meteor scores by 10.3\%. The Sure-Summ-BART pipeline model out-performs a baseline RoBERTa-BART pipeline model on all metrics.

%\asli{i think the faithfulness and diversity aspects should be motivated better. So far repeated summaries with extraction and abstraction method is great and implicitly one understand why it might work better over different metrics.}

%\asli{we need to stress the motivation here. For instance we claim we generate more factual and diverse, so stress here that extraction helps for faithfullness and abstraction for diversity or something.} 
%Moreover, \bartscore \cite{yuan2021bartscore} is used to evaluate faithfulness of the generated abstractive summary to the answers \asli{this is a very long sentence and not easy to understand}. Our supervised repeated-summarization model, which uses the gold relevant sentences during training, significantly improves upon the existing state-of-the-art model (BART) on faithfulness and diversity of generated summaries improving by 20\% on faithfulness scores, between 3.5\% - 5.8\% on Perspective scores, and by 5.4\% on Meteor scores while almost matching a strong BART baseline on Rouge scores. Note that we report significantly better Rouge scores for the BART baseline than the one in the Answersumm paper \cite{fabbri2021answersumm} owing to careful tuning of the model. In order to measure whether the gains are due to the additional intermediate supervision or the repeated summarization modeling, we also develop an unsupervised repeated-summarization model (UNSURE-Summ). This model does not use the gold relevant sentences and matches the BART model on Rouge scores. Moreover, it achieves relative improvement of 2.5\%,  3.3\%, and between 1.3\% to 3.5\% on Meteor scores, faithfulness scores, and Perspective scores respectively.


%\asli{This paragraph related to data, moved it futher down.}To make progress on this problem, \citet{fabbri2021answersumm} recently released the \answersumm{} dataset curated from StackExchange. Annotators were asked to extract relevant sentences from each answer for a question asked on the forum. They were then asked to cluster relevant sentences, generate cluster summaries, and finally combine the cluster summaries to produce a multi-perspective summary. Figure \ref{fig:example} shows an example instance from the dataset. In this paper, we focus on the \answersumm{} dataset to benchmark performance of state-of-the-art summarization models and develop novel models for this multi-perspective opinion summarization task. We make the following contributions in the paper.
%\input{tables/example_cluster_summaries}


%Next, through Oracle studies we show that relevant sentence selection can significantly improve summarization performance. However, accurately predicting relevant sentences is hard for opinionated data --- a carefully trained supervised Roberta model only achieves XXX\% Rouge score for relevant sentence selection while our multi-task model achieves XXX\% Rouge. However, given the observation that the BART baseline performs well when the number of perspectives is low, we demonstrate that relevant sentences in an answer can be leveraged to select the top few perspectives to pass to the BART model to further improve its performance. Towards this end we design a pipeline model that uses our multi-task model as a powerful relevant sentence predictor and an answer selection model coupled with the BART summarization model, all trained separately, to produce summaries that improve over the BART baseline by XXX\%. Furthermore, the pipeline model also improves median Rouge by XXX\% over all groups of examples with the same number of perspectives and is robust to changing the ordering of answers.

%Lastly, we rigorously investigate why passing all the answers as input to the BART model hurts performance. Towards this end we use information gain to demonstrate that many answers can have a negative effect (negative information gain) on the summary. Whereas it is easy for the model to ignore irrelevant answers which have zero information gain, including answers with negative information gain hurts summarization performance. 

%With the advent of large language models such as BART and Pegasus~\citet{}, abstractive summarization has recently improved dramatically.

%Unlike factoid  questions, in order to answer opinion-based queries, we may need to consider multiple perspectives. Not only the model should decide which perspectives to present but also it needs to present the possibly conflicting perspectives in a coherent way.


==> src/metrics_old.tex <==
\section{Metrics}
\subsection{Automatic Metrics}
To evaluate our models, we use ROUGE~\cite{lin-2004-rouge} for accuracy, METEOR \cite{banerjee2005meteor} for  \textit{multiperspectivity} and BARTScore~\cite{yuan2021bartscore} (as modified for our setting) for \textit{faithfulness}. 
Our analysis on using BERTScore~\cite{BERTScore} yielded saturated scores for our task where all models scored in excess of 95 F1-score.
See Appendix~\ref{app:autoevals} for details.

\subsubsection{Perspective Metric}
% The multi-perspective issue is a novel problem in summarization that existing automatic metrics fall short of capturing. 
In opinion-based summarization, the output summaries should reflect multiple representative perspectives rather than a single perspective. 
We introduce \emph{Perspective} metric, which uses the cluster annotations in the \answersumm{} dataset \cite{fabbri2021answersumm}. In \answersumm{}, relevant sentences from each answer are first clustered and each cluster is summarized before forming the final summary (see Fig. \ref{fig:full_example} in Appendix \ref{app:dataset_details} for an example).
We treat each cluster summary as one aspect that should be represented in the final summary and calculate the ROUGE score between each cluster summary and the generated summary. 
% As such, 
To determine if the cluster summary is represented in the generated summary, we use ROUGE Recall\footnote{ROUGE Precision is an alternative metric here though its value would be low since each cluster represents only one aspect of the final summary and is much shorter than it.} and average over all the cluster summaries to obtain the Perspective score:
\begin{equation}
    \textstyle \text{Perspective}= \frac{1}{N} \sum_i({\text{ROUGE}}_{\text{recall}}(y,S_i)),
\end{equation}
where $N$ is the total number of annotated clusters, $S_i$ is the summary of the $i^{th}$ cluster, and $y$ is the generates summary. Since we are using recall, the Perspective metric favors longer summaries. Hence, it needs to be used to compare models that have similar scores based on other metrics such as ROUGE which penalize long summaries. 

\subsubsection{A New Faithfulness Metric}
\label{anewfaithfullnessmetric}

\paragraph{Can BARTScore evaluate faithfulness of answer summarization tasks?}
Recent work shown improvements towards better evaluations of faithfulness or factual correctness of abstractive summaries \citep{surveyevaltextgen}. 
% Earlier works  ~\citet{falke2019ranking,gabriel-etal-2021-go} also show that that out-of-the-box entailment models trained on NLI datasets fail to evaluate factuality of the generated output summaries and do not correlate strongly with the ROUGE scores.
% A recent study by \citet{yuan2021bartscore} also shows that the log-likelihood scores of strong generative models like BART (referred to as \bartscore{} in their paper) can correlate well with human generated factuality scores. Specifically, they show that compared to the other metrics, the \bartscore{} (obtained from BART finetuned models on CNN dataset) correlates much strongly with the human factuality scores on the SummEval dataset (Table 4), as well as the summarization factuality datasets (i.e., Rank-19 and Q-CNN (Table 5)). 
However, we present several hypothesis and arguments in the next that even a state-of-the-art BARTScore has generalization issues when used on answer summarization model evaluations, hence we propose a new faithfulness evaluation score adapting the BARTScore.

We start with the BARTScore formulation by \citet{yuan2021bartscore}, which is defined as  `` \emph{direct evaluation of text through the lens of its probability of being generated}''. Formally, the faithfulness of a \emph{generator model} $f$ is computed by another seq2seq \emph{verifier model} $v$ as $\bs[v]{g(X); X} = \log p_v(f(X) \mid X)$, where $p_v(\parg)$ is the probability assigned by $v$ to a sequence.
Thus, it is crucial that the verifier model $v$ used for computing the \bartscore{} be a good \emph{generative model} as well so that its generation probabilities ($p_v(\parg)$) have high \emph{statistical power}. We claim that using the vanilla \bartscore{} won't be efficient for the answer summarization model evaluation since vanilla \bartscore{} is trained on news articles (i.e., CNN/DM datasets) while our models are trained and evaluated on the post about users answers to open domain questions (i.e., CQA data), which has a different discourse structure and semantic features compared to news datasets.  
% This is because cannot be used for our purpose due to the domain shift between news articles and CQA data. 
As suggested in \citet{yuan2021bartscore}, this domain shift issue can be mitigated by fine-tuning the underlying BART model on the task data which would then yield an enhanced \bartscore{} for the task at hand.  We should also note that the human annotators generate the reference summaries of multiple answers given a question by using only the relevant sentences from the answers. How can we build a verifier model that not only adapts the features of \bartscore{} but also evaluates the faithfulness of the multi-answer summarization task simulating human's evaluation criteria?

\noindent{\textbf{\bartscore{} for EA summarization.}} 
As we will show in the next section, we first build an Oracle BART model, by finetuning BART to generate the final summary from golden relevant sentences which are also used during inference. We use our Oracle BART model to compute an upper bound on various metrics and analyze different models. As predicted by Theorem \ref{thm:informal} a model that generates summaries from gold relevant sentences is always more faithful than a model that generates summaries from the original answers directly, when measuring faithfulness by log-likelihood scores.
Not surprisingly, we find that our Oracle BART model has by far the best performance across all metrics on the \answersumm{} dataset (Table \ref{tab:main_results}) including faithfulness.
This is intuitive since irrelevant sentences in the answer act as confounders which have been demonstrated to hurt performance in various settings like adversarial question answering  \cite{jia2017adversarial}. 

Denoting the \bartscore{} computed using the Oracle BART model as $\bs[\mathrm{OBART}]{\parg}$ we will measure the faithfulness of a model generated summary $g(X)$ with respect to the input as $\bs[\mathrm{OBART}]{g(X); Q, X}$. For the purpose of evaluating the faithfulness of abstractive summaries, we will assume that sentence level extractive summaries are faithful. We measure the faithfulness of the summary $g(X)$ generated by an EA model as $\bs[\mathrm{OBART}]{g(X); Q, R}$ where $R$ are the \textit{predicted relevant sentences}. In essence
the faithfulness metric serves to measure the faithfulness of the final summary with respect to the sentences that were actually used in generating the summary. By doing so we separate estimation of the factuality of the final (abstractive) summary from the quality of relevant sentences. A faithful summary does not indicate a relevant or useful summary. This also addresses the problem of long inputs which may exceed the maximum input length of the evaluator model. For more discussions see Appendix \ref{app:bart_score}.

\subsection{Human Evaluation}
% Finally, we also use human evaluation since automatic metrics have been shown to be inadequate in judging summarization quality as perceived by humans~\cite{maynez-etal-2020-faithfulness}. 
We conduct human evaluations and use multiple raters to evaluate summaries on a five point Likert scale along five axes: faithfulness, relevance, coherence, multiperspectivity, and overall quality. See Appendix \ref{app:human_eval} for details.


==> src/problem.tex <==
\section{Preliminaries}
We formalize the query-based answer summarization (QAS) problem as follows: Given a question $Q$, and a set of answers $X = \Set{X_1, \ldots, X_n}$ where each answer is a sequence of sentences, $X_{i,j} \in X_i$, QAS generates a summary $Y$ capturing different perspectives or opinions present in the answers.   Given $Q$, the answers $X_i$ are assumed to be independent of each other and the ordering of answers is not indicative of their importance in generating the summary. Optionally, in the supervised setting, each sentence $X_{i,j}$ in the training and validation set has a human annotated relevancy label $R_{i,j} \in \Set{0,1}$ indicating relevance of the sentence. To simplify the notation, we overload $R_i$ to denote either the set of relevant indicator labels or the set of relevant sentences in the i-th answer. 

When the dataset is generated following an annotation pipeline where human annotators first identify relevant sentences $R$ from $X$ and then only used the relevant sentences to generate the final summary $Y$ (e.g. \answersumm{} and \texttt{QMSUM} datasets), then true data distribution over answers, relevant sentences, and final summary follow a Markov process $X \rightarrow R \rightarrow Y$. The final summary $Y$ is conditionally independent of the input $X$ given relevant sentences $R$. Our first proposal is the following theoretical result concerning the performance of models generating $Y$ directly from $X$ versus generate it from $R$. See Appendix \ref{app:theoretical_result} for the formal statement of the theorem and the proof.

\begin{theorem}[Informal]
\label{thm:informal}
If the true data distribution over triples $(X, R, Y)$ 
is a Markov process $X \rightarrow R \rightarrow Y$, then the optimal predictor trained to generate $Y$ from $X$ can never outperform the optimal predictor trained to generate $Y$ from $R$, when performance of a predictor is measured by the log-likelihood of the predictions under the true data distribution. 
\end{theorem}
%\asli{what if X $\sim$, then Y can be easily generated from X (by copying) without the need for R? Or if X is very similar to R, or all information in X is salient for instance? If the relevant sentences are awalys the first sentences and the model learns to select the first sentence from each sentence, then do we still need R?}
The above information-theoretical result is applicable to any data distribution with the aforementioned Markovian property (including but not limited to EA summarization) no matter how adversarially $R$ is generated from $X$ and $Y$ from $R$, when using expressive predictor function classes (e.g., neural networks with enough capacity).


==> tables/gold_vs_distant_relevant.tex <==
\begin{table}[]
    \centering
    \resizebox{\linewidth}{!}{%
    \begin{tabular}{c | c | ccc@{} | cc c@{} | cc @{}c@{}|}
        \multicolumn{2}{c}{} & \multicolumn{8}{c}{automatic} & \multicolumn{1}{c}{} \\ 
        \cline{2-11}   
        & & \multicolumn{2}{c}{$\tau=0.12$} & & \multicolumn{2}{c}{$\tau=0.14$} && \multicolumn{2}{c}{$\tau=0.2$} & \\
        & & 0 & 1 & & 0 & 1 & & 0 & 1 & \\
        \cline{2-11}
        \multirow{2}{*}{gold} & 0 & 0.55 & 0.45 & & 0.64 & 0.36 & & 0.84 & 0.16 & \\
        & 1 & 0.29 & 0.71 & & 0.37 & 0.63 & & 0.61 & 0.39 & \\
        \cline{2-11}        
    \end{tabular}}
    \caption{Probability that sentence is relevant as computed using distant supervision (automatic)
    given that sentence is marked as relevant by humans (gold), i.e., $\Prob{\mathrm{ROUGE}\_1(X_{i,j}, Y) \geq \tau \mid R_{i,j} = 1} = 0.71$ for $\tau = 0.12$.}
    \label{tab:gold_vs_distant}
\end{table}









==> tables/human_eval_results.tex <==
\begin{table}
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{cccccc}
\hline    
& Fai. & Rel. & Mul. & Coh. & Qua. \\
\hline
Oracle BART &  4.0 & 4.4 & 3.1 & 4.5 & 3.5 \\
RoBERTa-BART &  3.9 & 4.4 & 4.2 & 4.3 & 3.7 \\
SURE-Summ-BART  & 3.8 & 4.2 & 3.2 & 4.3 & 3.4 \\
SURE-Summ &  3.9 & 4.1 & 3.1 & 4.2 & 3.4 \\
UNSURE-Summ-BART & 3.8 & 4.3 & 2.8 & 4.5 & 3.3 \\
UNSURE-Summ &  3.9 & 4.3 & 3.1 & 4.2 & 3.5 \\
BART &  3.9 & 4.5 & 2.9 & 4.3 & 3.4 \\
\hline
\end{tabular}}
\caption{Human evaluation results along different axes: Faithfulness, Relevance, Multiperspectivity, Coherence, Overall Summary Quality.}
\label{tab:human_eval_results}
\end{table}


==> tables/main_results.tex <==
\begin{table*}[htbp]
    \centering
    \begin{tabular}{cccccc}
        \hline
        Method & \#Params & F1 Rouge 1/2/L & Meteor & Faithfulness & Perspective 1/2/L \\
        \hline
        \hline
        \multicolumn{6}{c}{Oracle models} \\
        \hline        
        Sup. Oracle BART & 406M & 34.2 / 11.6 / 23.9 & 24.4 & -87.1 & 45.6 / 15.4 / 36.3 \\
        Unsup. Oracle BART & 406M & 33.3 / 10.9 / 23.3 & 22.5 & -146.1 & 41 / 12.8 / 32.8 \\
        \hline
        BART & 406M & 30.2 / 9.2\td / \textbf{21.3} & 20.3 & -156.9 & 39.7 / 11.3 / 31.5 \\
        T5  & & ?? & ?? & ?? & ?? \\
        SURE-Summ & 406M & 30.2 / 8.9 / 20.8 & 21.4\td & -125.6\td & 42\td / 11.7\td / 33\td \\
        UNSURE-Summ & 406M & 30.3\td / 9.0 / 21.2 & 20.8 & -151.8 &  40.5 / 11.7 / 31.9 \\
        \hline
        \multicolumn{6}{c}{Pipeline models}\\
        \hline
        Sup. RoBERTa-BART & 761M & 30.6 / 9 / 20.9 & 22 & -86 & 44 / 12.7 / 34.5 \\
        SURE-Summ-BART & 812M & {\bf 30.8} / {\bf 9.3} / 21.1 & {\bf 22.4} & {\bf -79.9} & {\bf 44.2} / \textbf{13.2} / \textbf{34.8} \\
        UNSURE-Summ-BART & 812M & 30 / 9.2 / \textbf{21.3} & 20.2 & -147.9 & 38.7 / 11 / 30.6 \\
        \hline
    \end{tabular}
–––    \caption{Performance of different methods on the test set of the \answersumm{} 
    data set. Oracle models refer to models which have access to the gold (Sup. BART) 
    or distantly supervised (Unsup. BART) relevant sentence labels during inference.
    Pipeline models refer to models where the extractor and generator models are trained
    separately.}
    \label{tab:main_results}
\end{table*}

==> tables/main_results_unsupervised.tex <==
\begin{table*}[htbp]
    \centering
    \small
    \resizebox{\linewidth}{!}{%
    \begin{tabular}{ccccccc}
        \hline
        Method & \#Params & F1 Rouge 1/2/L & Meteor & Faithfulness & Perspective 1/2/L & Length \\
        \hline
        \hline
        \multicolumn{7}{c}{Oracle models} \\
        \hline        
        Sup. Oracle BART & 406M & 34.2 / 11.6 / 23.9 & 24.4 & -87.1 & 45.6 / 15.4 / 36.3 & 214 \\
        Unsup. Oracle BART & 406M & 33.3 / 10.9 / 23.3 & 22.5 & -146.1 & 41 / 12.8 / 32.8 &  178 \\
        \hline
        \multicolumn{7}{c}{Supervised models} \\
        \hline
        BART-rel & 406M & 29.9 / 8.5 / 20.5 & 21.3 & -89.7 & 43.6 / 12.4 / 34.1 & 242 \\
        SURE-Summ & 406M & 30.2 / 8.9 / 20.8 & 21.4 & -125.6 & 42 / 11.7 / 33 & 215 \\        
        Sup. RoBERTa-BART & 761M & 30.6\td / 9\td / 20.9\td & 22\td & -86\td & 44\td / 12.7\td / 34.5\td & 242 \\
        SURE-Summ-BART & 812M & {\bf 30.8} / {\bf 9.3} / \textbf{21.1} & {\bf 22.4} & {\bf -79.9} & {\bf 44.2} / \textbf{13.2} / \textbf{34.8} & 240 \\
        \hline
        \multicolumn{7}{c}{Unsupervised models}\\
        \hline
        BART & 406M & 30.2\td / \textbf{9.2} / \textbf{21.3} & 20.3 & -156.9 & 39.7 / 11.3 / 31.5 & 184 \\
        PEGASUS & 568M & 29.6 / 8.8 / 20.7  & 20.4 & -153.8 & 39.7 / 11.5 / 31.6 & 198 \\
        T5  & 220M & 29.5 / 8.8 / 20.6 & 20.6\td & -201.8 & \textbf{40.8} / \textbf{12} / \textbf{32.5} & 218 \\
        UNSURE-Summ & 406M & \textbf{30.3} / 9.0\td / 21.2\td & \textbf{20.8} & -151.8\td & 40.5\td / 11.7\td / 31.9\td & 187 \\  
        UNSURE-Summ-BART & 812M & 30 / \textbf{9.2} / \textbf{21.3} & 20.2 & \textbf{-147.9} & 38.7 / 11 / 30.6 & 179 \\
        \hline
    \end{tabular}}
    \vspace{-0.2cm}
    \caption{\small Performance of different methods on the test set of the \answersumm{} 
    data set. Oracle models refer to models which have access to the gold (Sup. Oracle BART) 
    or distantly supervised (Unsup. Oracle BART) relevant sentence labels during inference.
    Pipeline models refer to models where the extractor and generator models are trained
    separately.}
    \label{tab:main_results}
\end{table*}

==> tikz.tex <==
\usepackage{tikz}
\usetikzlibrary{arrows}
\usetikzlibrary{shapes}
\usetikzlibrary{decorations.pathreplacing}
\usetikzlibrary{shapes.misc, positioning, quotes}
\usetikzlibrary{patterns}

\makeatletter
\def\grd@save@target#1{%
  \def\grd@target{#1}}
\def\grd@save@start#1{%
  \def\grd@start{#1}}
\tikzset{
  grid with coordinates/.style={
    to path={%
      \pgfextra{%
        \edef\grd@@target{(\tikztotarget)}%
        \tikz@scan@one@point\grd@save@target\grd@@target\relax
        \edef\grd@@start{(\tikztostart)}%
        \tikz@scan@one@point\grd@save@start\grd@@start\relax
        \draw[minor help lines] (\tikztostart) grid (\tikztotarget);
        \draw[major help lines] (\tikztostart) grid (\tikztotarget);
        \grd@start
        \pgfmathsetmacro{\grd@xa}{\the\pgf@x/1cm}
        \pgfmathsetmacro{\grd@ya}{\the\pgf@y/1cm}
        \grd@target
        \pgfmathsetmacro{\grd@xb}{\the\pgf@x/1cm}
        \pgfmathsetmacro{\grd@yb}{\the\pgf@y/1cm}
        \pgfmathsetmacro{\grd@xc}{\grd@xa + \pgfkeysvalueof{/tikz/grid with coordinates/major step}}
        \pgfmathsetmacro{\grd@yc}{\grd@ya + \pgfkeysvalueof{/tikz/grid with coordinates/major step}}
        \foreach \x in {\grd@xa,\grd@xc,...,\grd@xb}
        \node[anchor=north] at (\x,\grd@ya) {\pgfmathprintnumber{\x}};
        \foreach \y in {\grd@ya,\grd@yc,...,\grd@yb}
        \node[anchor=east] at (\grd@xa,\y) {\pgfmathprintnumber{\y}};
      }
    }
  },
  minor help lines/.style={
    help lines,
    step=\pgfkeysvalueof{/tikz/grid with coordinates/minor step}
  },
  major help lines/.style={
    help lines,
    line width=\pgfkeysvalueof{/tikz/grid with coordinates/major line width},
    step=\pgfkeysvalueof{/tikz/grid with coordinates/major step}
  },
  grid with coordinates/.cd,
  minor step/.initial=.2,
  major step/.initial=1,
  major line width/.initial=1pt,
}
\makeatother


%\newcommand{\tikzhelplines}[2]{
%     \draw (#1) to[grid with coordinates] (#2);
%}

